Spatio-Temporal-based Context Fusion for Video Anomaly Detection

Video anomaly detection aims to discover abnormal events in videos, and the principal objects are target objects such as people and vehicles. Each target in the video data has rich spatio-temporal context information. Most existing methods only focus on the temporal context, ignoring the role of the spatial context in anomaly detection. The spatial context information represents the relationship between the detection target and surrounding targets. Anomaly detection makes a lot of sense. To this end, a video anomaly detection algorithm based on target spatio-temporal context fusion is proposed. Firstly, the target in the video frame is extracted through the target detection network to reduce background interference. Then the optical flow map of two adjacent frames is calculated. Motion features are used multiple targets in the video frame to construct spatial context simultaneously, re-encoding the target appearance and motion features, and finally reconstructing the above features through the spatio-temporal dual-stream network, and using the reconstruction error to represent the abnormal score. The algorithm achieves frame-level AUCs of 98.5% and 86.3% on the UCSDped2 and Avenue datasets, respectively. On the UCSDped2 dataset, the spatio-temporal dual-stream network improves frames by 5.1% and 0.3%, respectively, compared to the temporal and spatial stream networks. After using spatial context encoding, the frame-level AUC is enhanced by 1%, which verifies the method's effectiveness.

==> Spatio-Temporal-based Context Fusion for Video Anomaly Detection/mir-sample-bib.tex <==
\begin{thebibliography}{9}



\bibitem{bib1} B. Ran, D. E. Boyce. {\sl Modeling Dynamic Transportation Network}, Berlin, Germany: Springer-Verlag, pp. 69-83,1996. (Book style)

\bibitem{bib2} G. O. Young. Synthetic structure of industrial plastics. Plastics, 2nd ed., J. Peters, Ed., New York, USA: McGraw-Hill, pp. 15-64, 1964. (Book style with paper title and editor)

\bibitem{bib3} L. C. Su, F. Zhu. Design of a novel omnidrectional stereo vision system. {\sl Acta Automatica Sinica}, vol. 32, no. 1, pp. 67-72, 2006. (in Chinese) (Periodical style)

\bibitem{bib4} R. Roychoudhury, S. Bandyopadhyay, K. Paul. Adistributed mechanism for topology discovery in ad hoc wireless networks using mobile agents. In {\sl Proceedings of IEEE First Annual Workshop on Mobile and Ad hoc Networking and Computing}, IEEE, Piscataway, USA, pp. 145-146,2000. (Published Conference Proceedings style)

\bibitem{bib5} O. Hryniewicz. An evaluation of the reliability of complex systems using shadowed sets and fuzzy lifetime data. {\sl International Journal of Automation and Computing}, to be published.

\bibitem{bib6} W. Zhang. Reinforcement Learning for Job-shop Scheduling, Ph. D. dissertation, Oregon State University, USA,1996. (Dissertation style)

\bibitem{bib7} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969. (Standards style)

\bibitem{bib8} R. C. Reily, J. L. Mack. The Self-organization of Spatially Invariant Representations, Technical Report PDP. CNS.92.5, Department of Psychology, Mellon University, USA, 1993. (Report style)

\bibitem{bib9} J. P. Wilkinson. Nonlinear Resonant Circuit Devices, U.S. Patent 362412, July 1990. (Patent style)

\bibitem{bib10} J. Jones. {\sl Networks}, 2nd ed., [Online], Available: http://www.atm.com, May 10, 1991.

\bibitem{bib11} R. J. Vidmar. On the use of atmospheric plasmas as electromagnetic reflectors. {\sl IEEE Transactions on Plasma Science}, vol. 21, no. 3, pp. 945-999, [Online], Available: http://www.halcyon.com, July 20-25, 1999.



\end{thebibliography}



==> mir-sample-bib.tex <==
\begin{thebibliography}{9}



\bibitem{bib1} B. Ran, D. E. Boyce. {\sl Modeling Dynamic Transportation Network}, Berlin, Germany: Springer-Verlag, pp. 69-83,1996. (Book style)

\bibitem{bib2} G. O. Young. Synthetic structure of industrial plastics. Plastics, 2nd ed., J. Peters, Ed., New York, USA: McGraw-Hill, pp. 15-64, 1964. (Book style with paper title and editor)

\bibitem{bib3} L. C. Su, F. Zhu. Design of a novel omnidrectional stereo vision system. {\sl Acta Automatica Sinica}, vol. 32, no. 1, pp. 67-72, 2006. (in Chinese) (Periodical style)

\bibitem{bib4} R. Roychoudhury, S. Bandyopadhyay, K. Paul. Adistributed mechanism for topology discovery in ad hoc wireless networks using mobile agents. In {\sl Proceedings of IEEE First Annual Workshop on Mobile and Ad hoc Networking and Computing}, IEEE, Piscataway, USA, pp. 145-146,2000. (Published Conference Proceedings style)

\bibitem{bib5} O. Hryniewicz. An evaluation of the reliability of complex systems using shadowed sets and fuzzy lifetime data. {\sl International Journal of Automation and Computing}, to be published.

\bibitem{bib6} W. Zhang. Reinforcement Learning for Job-shop Scheduling, Ph. D. dissertation, Oregon State University, USA,1996. (Dissertation style)

\bibitem{bib7} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969. (Standards style)

\bibitem{bib8} R. C. Reily, J. L. Mack. The Self-organization of Spatially Invariant Representations, Technical Report PDP. CNS.92.5, Department of Psychology, Mellon University, USA, 1993. (Report style)

\bibitem{bib9} J. P. Wilkinson. Nonlinear Resonant Circuit Devices, U.S. Patent 362412, July 1990. (Patent style)

\bibitem{bib10} J. Jones. {\sl Networks}, 2nd ed., [Online], Available: http://www.atm.com, May 10, 1991.

\bibitem{bib11} R. J. Vidmar. On the use of atmospheric plasmas as electromagnetic reflectors. {\sl IEEE Transactions on Plasma Science}, vol. 21, no. 3, pp. 945-999, [Online], Available: http://www.halcyon.com, July 20-25, 1999.



\end{thebibliography}


